Torische Ideale von Flusspolytopen

In dieser Diplomarbeit werden einige Gradschranken f\"ur Erzeugendensysteme und Gr\"obnerbasen von torischen Idealen von Flusspolytopen bewiesen. Alle torischen Ideale von Flusspolytopen sind im Grad 3 erzeugt. Glatte (3x4)-Transportpolytope sind sogar im Grad 2 erzeugt. Die reduzierte Gr\"obnerbasis eines beliebigen (m \times n)-Transportpolytops bez\"uglich einer beliebigen umgekehrt lexikographischen Termordnung hat h\"ochstens Grad mn/2. Wir konstruieren auch ein Beispiel, f\"ur das diese Schranke ann\"ahernd scharf ist. ----- In this Diplomarbeit (Master's thesis), we prove some degree bounds for generating sets and Gr\"obner bases of toric ideals of flow polytopes. All toric ideals of flow polytopes are generated in degree three. Smooth (3x4)-transportation polytopes are even generated in degree 2. The reduced Gr\"obner basis of an arbitrary (m \times n)-transportation polytope with respect to an arbitrary reverse lexikographic term order has at most degree mn/2. We also construct an example, for which this bound is almost sharp.

==> 3xnZellenkubisch.tex <==

%
%
%
%

\section{$3 \times n$-Zellen}

In diesem Abschnitt soll gezeigt werden, dass alle Grad drei Relationen vom Birkhoff-Typ sind und dass
Relationen vom Grad größer gleich vier gar nicht auftreten.

Im nächsten Schritt in ferner Zukunft soll dann auch gezeigt werden, dass man Birkhoff-Relationen
immer retten kann.

In noch fernerer Zukunft sollen diese Ergebnisse dann auf größerem Zellen ($4 \times n$, $m \times n$) verallgemeinert werden.

\subsection{Begriffe, Grundlagen}
Wir betrachten nun Zellen $Z$ eines $3 \times n$-Transportpolytops mit Zeilensummen
$1\le r_1 \le r_2 \le r_3 \le n-1$ und Spaltensummen
$1 \le c_1 \le \ldots \le c_n \le 2$. Mit $A_j$ bezeichnen wir die $j$-te Spalte einer Matrix $A$.

\begin{Definition}[Relation]
Eine Relation $R$ vom Grad $r$ ist eine Familie $\{M^1,\ldots, M^r, N^1, \ldots, N^r\}$ ($M^i, N^i \in Z$) mit
$ \sum_i M^i = \sum_i N^i$.
\end{Definition}

\begin{Definition}
Eine Menge von Relationen $R_1, \ldots, R_l$ erzeugt $R$ wenn es $z,z_1,\ldots, z_l \in \Z_{\ge 0}$ gibt
mit $zR = \sum_i z_iR_i$. 
\end{Definition}

\begin{Bemerkung}
Diese Definition entspricht der algebraischen Version.
\end{Bemerkung}


\begin{Definition}[Fixspalten]
Sei $V \subseteq [n]$. Eine Relation $R$ heißt fix auf $V$, wenn für alle $j \in V$ gilt:
$ M^1_j = M^2_j = M^3_j  = M^4_j =  N^1_j = N^2_j = N^3_j = N^4_j $, dass heißt die Spalten aus $V$ sind bei allen beteiligten Matrizen gleich.
\end{Definition}

\begin{Lemma}
\label{Aufteilungslemma}
Es gebe $n_1,n_2 \in \N$ mit $n_1 + n_2 = n$ und Permutationen $\sigma_2, \ldots \sigma_r, \tau_1, \ldots \tau_r \in S_{n_1} \times S_{n_2}$, sodass $M^i=\sigma_i M^1$ und $N^i=\tau_i M^1$, d.h man kann die Matrizen ineinander überführen, indem man die ersten $n_1$ und die letzten $n_2$ Vektoren untereinander permutiert.
Dann lässt sich $R$ durch Relationen darstellen, die fix auf $\{1,\ldots, n_1\}$ sind und durch solche, die
fix auf $\{n_1+1,\ldots, n\}$ sind.
\end{Lemma}
\begin{proof}
Betrachte die Relation $R$ mit ${\sum_i}  M^i = {\sum_i}  N^i$.
Es sei $M^i = [\bar{M}^i|\tilde{M}^i]$ und $N^i = [\bar{N}^i|\tilde{N}^i]$.
Dann gilt offensichtlich:
\begin{eqnarray}
\label{relA}
\sum_i [\bar{M}^i|\tilde{M}^j] &=& \sum_i [\bar{N}^i|\tilde{N}^j] \\
\label{relB}
\sum_j [\bar{M}^i|\tilde{M}^j] &=& \sum_j [\bar{N}^i|\tilde{N}^j] 
\end{eqnarray}
Diese $2n$ Relationen erzeugen $R$. Es gilt nämlich:
\begin{eqnarray}
n \sum_i [\bar{N}^i|\tilde{N}^i] 
&=&
\sum_i \sum_j [\bar{N}^i|\tilde{N}^j] \\
&\gleich{(*)}&
\sum_i \sum_j [\bar{M}^i|\tilde{M}^j] \\
&=&
n \sum_i [\bar{M}^i|\tilde{M}^i] 
\end{eqnarray}
Gleichheit bei $(*)$ erhält man durch Aufsummieren von \label{relA} und \label{relB}
für alle $i,j$.

\end{proof}


\begin{Korollar}
Es genügt also nur den Fall zu betrachten, dass alle Spaltensummen 1 sind.
Der Spaltensummen 2 Fall kann aufgrund des obigen Lemmas getrennt behandelt werden, ist aber komplett symmetrisch dazu.
\end{Korollar}

\begin{Definition}[Schnittspalten]
Sei $R$ eine Relation und $A,B$ seien Matrizen, die in dieser Relation vorkommen. Die $j-te$ Spalte heißt \emph{Schnittspalte} von $A$ und $B$, wenn $A_j=B_j$ gilt.
\end{Definition}


\begin{Definition}[Relationstyp]
Betrachte eine Relation $R$. $\Sigma_R := \sum_i M^i = \sum_i N^i$
nennen wir den Typ der Relation.

\end{Definition}


\begin{Definition}[Spaltentyp/Spaltenklasse]
Wir betrachten eine Relation $R$ vom Typ $\Sigma_R$. Wir nennen 
${\Sigma_R}_j$ den Typ der $j$-ten Spalte. 
Die Menge der Spaltenklassen in $3\times n$-Zellen einer Relation vom Grad $r$ bezeichnen wir mit $T_{r}$. Es gilt
$T_{r}=\{( s_1,s_2,s_3)\in \N^3 :  s_1 + s_2 + s_3 = r\}$.

Betrachte die Relation $\sim$ auf der Menge der Spaltentypen mit $t_1 \sim t_2 \Leftrightarrow
\exists \sigma \in S_3 : \sigma t_1=t_2$. Dann definieren wir die Menge der Spaltenklassen $K_r := T_r/\sim$
\end{Definition}


\subsection{Tauschlemmata}
In diesem Abschnitt werden einige Lemmata bewiesen, die es ermöglichen, Relationen durch andere darzustellen.
\begin{Lemma}[1. Tauschlemma]
Betrachte eine Relation $R$ vom Grad $r$. Sei $a,b$ Schnittspalten von $M_i$ und $N_j$ (o.B.d.A sei $i=j=r$.
Dann wird $R$ erzeugt von 
\begin{eqnarray*}
\sum_i^{r-1} M^i + \tilde{M}^i &=& \sum_i^{r-1} N^i + \tilde{N}^n
\\
M^n + \tilde{N}^n &=& N^n + \tilde{M}^n 
\end{eqnarray*}
\end{Lemma}
\begin{proof}
Klar.
\end{proof}
Man kann auch innerhalb einer Seite der Relation tauschen, wie die beiden folgenden Lemmata zeigen:
\begin{Lemma}[2. Tauschlemma]
Sei $M^1_i=M^2_j$ und $M^1_j=M^2_i$.
Definiere $\tilde{M^1}=(i j)M^1$ und $\tilde{M^2}=(i j)M^2$. Dann erzeugen

\begin{eqnarray*}
\tilde{M^1} + \tilde{M^2} + \sum_{i=3}^r M^i &=& \sum_{i=1}^r N^i \\
\tilde{M^1} + \tilde{M^2} & = & M^1 + M^2 
\end{eqnarray*}
die Relation $R$.
\end{Lemma}
\begin{proof}
Klar.
\end{proof}

\begin{Lemma}[Birkhoff-Tausch]
Betrachte eine Relation $R$ mit:
\begin{eqnarray}
M_1 =
\begin{bmatrix}
1 0 0 \\
0 1 0 & X_1 \\
0 0 1 
\end{bmatrix}
\quad
&
M_1 =
\begin{bmatrix}
0 0 1 \\
1 0 0 & X_2 \\
0 1 0 
\end{bmatrix}
\quad
&
M_1 =
\begin{bmatrix}
0 1 0 \\
0 0 1 & X_3 \\
1 0 0 
\end{bmatrix}
\end{eqnarray}
Dann kann man $M^1, M^2, M^3$ ersetzen durch $\tilde{M^1}, \tilde{M^2}, \tilde{M^3}$ mit
\begin{eqnarray}
M_1 =
\begin{bmatrix}
1 0 0 \\
0 0 1 & X_1 \\
0 1 0 
\end{bmatrix}
\quad
&
M_1 =
\begin{bmatrix}
0 1 0 \\
1 0 0 & X_2 \\
0 0 1 
\end{bmatrix}
\quad
&
M_1 =
\begin{bmatrix}
0 0 1 \\
0 1 0 & X_3 \\
1 0 0 
\end{bmatrix}
\end{eqnarray}

\end{Lemma}
\begin{proof}
Klar.
\end{proof}

\begin{Lemma}[Großes Tauschlemma]
Sei $R$ eine Relation vom Grad vier.
Dann wird $R$ erzeugt von 
\begin{eqnarray*}
S_1 + M_1 + M_2 &=& T_1 + N_1 + N_2 \\
S_2 + M_3 + M_4 &=& T_2 + N_3 + N_4 \\
S_1 + S_2 &=&  T_1 + T_2 
\end{eqnarray*}
\end{Lemma}
\begin{Bemerkung}
Beweis wieder klar. Wenn man diese $S_i, T_i$ immer finden könnte, wäre man in einem Schlag fertig. Aber ob das geht ist fraglich.
Verallgemeinern kann man das offensichlich auf beliebige Relationen mit $r$ gerade und irgendwie sicher auch auf solche mit $r$ ungerade.
\end{Bemerkung}

\begin{Lemma}[Schubfachlemma]
Sei $r_3 \ge r_1 + r_2$.  Dann kann man eine $e_§$ Spalte gegen eine $e_1$ oder $e_2$ Spalte tauschen. Und zwar so:
OBdA sei: $M^1_1 = N^1_1 = e_2$. Dann existiert ein $j \not=1$ mit $M^1_j=N^1_j$, man kann also tauschen.
\end{Lemma}
\begin{proof}
Nach Voraussetzung ist $r_3 \ge \frac n 2$. In der letzten Zeile von $M_1$ und $N_2$ stehen also in den Spalten $2,\ldots, n$ (n-1 Stück) mehr als $\frac n 2$ Einsen. Nach Schubfachprinzip muss also in einer Spalte bei beiden Matrizen eine 1 stehen.
\end{proof}

Wir müssen uns im folgenden also nur noch um Zellen kümmern mit $r_3 < r_1 + r_2$.

\subsection{Grad 3 Relationen sind vom Birkhoff-Typ}
Idee war:

Klasse (2,1,0) kann man mit 1. Tauschlemma retten. Der Beweis dafür hat sich aber als falsch rausgestellt.

Wenn man nur Typ (1,1,1) zerlegt sich die Relation in viele disjunkte Birkhoffrelationen, die kann man nach
\ref{Aufteilungslemma} alle einzeln abhandeln.

\subsection{Grad 4 Relationen gibt es nicht}
Es gibt die Klassen (0,0,4), (0,1,3), (0,2,2), (1,1,2).
Die erste klasse ist Super. Die dritte kann man tauschen (s.u.)
bei der zweiten dachte ich auch, man könne sie tauschen, der Beweis ging dann aber nicht (wie bei Birkhoff).
Wenn es nur noch die 4. gibt kann man einen Grad 2 Binnentausch machen.

\begin{Lemma}
Sei die erste Spalte vom Typ (0,2,2). Dann kann man tauschen.
\end{Lemma}
\begin{proof}
Sei $M^1_1=N^1_1=M^2_1 = N^2_1 = e_2$ und $M^1_1=N^1_1=M^2_1 = N^2_1 = e_3$.
Wir müssen zeigen, dass es $i,j \in \{1,2\}$ und $k\in \{2,\ldots, n\}$ gibt mit
$M^i_k = N^j_k$, denn dann kann man tauschen.

Dieser Beweis von mir geht auch nicht durch.

\end{proof}

Gibt es nur Spalten vom Typ (2,1,0), so kann man mit Fallunterscheidungen erreichen, dass das Zweierbinnentauschlemma angewendet werden kann.

\begin{Bemerkung}
Also alles in allem eine recht traurige Situation. Die Aussage scheint zu stimmen, in allen Beispielen, die ich angeschaut habe. 3x10 Zellen kann der Rechner schon nicht mehr komplett überprüfen.
Aber in jedem Spezialfall muss man erst lange rumfriemeln, bis man es hat.
Meine bisherigen Beweisversuche benutzen die Struktur noch nicht richtig aus. Das wird sich im neuen Jahr hoffentlich ändern.

Frohe Weihnachten!
\end{Bemerkung}


==> Triangulierungen.tex <==

\section{Triangulierungen}

\begin{Definition}[polyedrische Komplexe]
 Ein \emph{polyedrischer Komplex} ist eine Menge $\Delta$ von Polyedern im $\R^d$ für die gilt:
\begin{itemize}
 \item $P\in\Delta, Q\seite P\Rightarrow Q\in\Delta$
 \item $P,Q\in \Delta\Rightarrow P\cap Q\seite P$
Falls alle Elemente von $\Delta$ Polytope sind, so nenne ich $\Delta$ einen \emph{polytopalen Komplex} und falls alle Elemente Kegel sind, so wird $\Delta$ mit \emph{Fächer} bezeichnet.

\end{itemize}
\end{Definition}

\begin{Definition}[Träger]
Sei $\Delta$ ein polyedrischer Komplex. Der \emph{Träger} von $\Delta$ ist definiert als:
\[|\Delta|:=\bigcup_{P\in \Delta} P\] 
\end{Definition}


\begin{Definition}[Unterteilungen und Triangulierungen]

Ein polyedrischer Komplex $\Delta'$ mit $|\Delta'|=|\Delta|$ ist eine Unterteilung von $\Delta$, 
falls es für alle $P\in \Delta'$ ein $Q\in \Delta$ gibt mit $P\subseteq Q$.

Falls alle Elemente von $\Delta'$ Simplexe bzw. simplizale Kegel sind, so heißt $\Delta'$ \emph{Triangulierung} von $\Delta$ (s. Abbildung \ref{figure:Triangulierungen})

 
\end{Definition}


\begin{figure}[!ht]
\centering
\subfloat[Im $\R^2$ haben alle Polytope unimodulare Triangulierungen]
{

\scalebox{0.4}{
	\input{TriangulierungPolygon.pstex_t}

} 

}
\hspace*{2mm}
\subfloat[Pulling-Tri\-an\-gu\-lie\-rung eines Polygons]
{

\scalebox{0.4}{
		\input{PullingTriangulierungPolygon.pstex_t}
}

}
\hspace*{1mm}
\subfloat[Diese Triangulierung ist nicht unimodular]
{

\scalebox{0.53}{
	\input{NichtUnimodularWuerfel2.pstex_t}
	} 
}

%
\caption{Drei Triangulierungen}
\label{figure:Triangulierungen}

\end{figure}





Sei $P$ ein Polytop und $v$ eine Ecke von $P$, sowie $\Delta$ ein polytopaler Komplex mit $|\Delta|=P$. Dann definieren erhalten wie folgendermaßen eine Unterteilung $\pull(P,v)$ von $\Delta$: Sei $Q\in\Delta$. Für $v\not\in Q$ sei $Q\in\pull(P,v)$.
Für $v\in Q$, $v\not\in Q'\subset Q$ sei $\conv(Q',v)\in\pull(P,v)$. Bildlich erhält man diese neue Unterteilung, indem man an der Ecke $v$ zieht.

Wie man leicht sieht erhält man so tatsächlich wieder eine Unterteilung. 
Auf analoge Weise kann man auch einen Fächer unterteilen (dann fügt man statt
dem Polytop$\conv(Q',v)$ den Strahl $Q'+v$ hinzu).
Zieht man nacheinander an allen Ecken des Polytops, so erhält man eine Triangulierung des Polytops, die für uns günstige Eigenschaften hat.
 


Dies fassen wir in der folgenden Definition zusammen.
\begin{Definition}[Pulling-Triangulierung]
Sei $P$ ein Polytop und $\Delta$ eine Unterteilung von $P$. 
$\pull$ .. ist dann triangulierung.
\end{Definition}




Man kann Simplizialkomplexe und Triangulierungen auch rein kombinatorisch definieren. 

Ein Simplizialkomplex auf einer Menge $V$ ist eine Menge $\emptyset\not=\Delta\subseteq \pot(V)$ mit $\sigma\in\Delta, \tau\subseteq \sigma \Rightarrow \tau\in \Delta$. 

Eine Triangulierung eines Polytops liefert einem dann einen kombinatorischen Simplizialkomplex auf der Menge der $\A=\{\vek{a}_1,\ldots,\vek{a}_n\}$ der Gitterpunkte von $P$.

Da diese Darstellungen beide äquivalent sind werde ich regelmäßig zwischen ihnen hin- und herspringen und die für den jeweiligen Fall günstigste verwenden. Manchmal werde ich auch die Menge $\A$ der Einfachheit halber auch mit der Menge $[n]$ identifizieren. 

Sei $\Delta$ ein Simplizialkomplex auf $[n]$ und $A\subseteq[n]$. Wenn $A\in\Delta$ gilt, so heißt $A$ \emph{Seite} von $\Delta$, andernfalls Nicht-Seite.

%
%
%
  







\begin{figure}[!ht]
\centering
\subfloat[An der markierten Ecke wird gezogen]
{

\scalebox{0.4}{
	\input{PullingWuerfel1.pstex_t}
} 

}
\subfloat[Nachher]
{

\scalebox{0.4}{
	\input{PullingWuerfel2.pstex_t}}
\hspace*{2mm}
\scalebox{0.4}{
	\input{PullingWuerfel3.pstex_t}
	} 
}
%
\caption{Pullingtriangulierung eines Würfels}
\label{figure:PullingWuerfel}
\end{figure}



Sei $P$ ein Polytop und $v$ eine Ecke von $P$, sowie $\Delta$ ein polytopaler Komplex mit $|\Delta|=P$. Dann definieren erhalten wie folgendermaßen eine Unterteilung $\pull(P,v)$ von $\Delta$: Sei $Q\in\Delta$. Für $v\not\in Q$ sei $Q\in\pull(P,v)$.
Für $v\in Q$, $v\not\in Q'\subset Q$ sei $\conv(Q',v)\in\pull(P,v)$. Bildlich erhält man diese neue Unterteilung, indem man an der Ecke $v$ zieht.
(siehe Abbildung \ref{figure:PullingWuerfel})


Wie man leicht sieht erhält man so tatsächlich wieder eine Unterteilung. 
Auf analoge Weise kann man auch einen Fächer unterteilen (dann fügt man statt
dem Polytop$\conv(Q',v)$ den Strahl $Q'+v$ hinzu).
Zieht man nacheinander an allen Ecken des Polytops, so erhält man eine Triangulierung des Polytops, die die für uns günstige Eigenschaften hat, dass sie unter bestimmten Voraussetzungen stets unimodular ist, was später bewiesen wird (s. Pacos Lemma).


\begin{Definition}[Pulling-Triangulierung]
Sei $R=(r_1,\ldots,r_k)$. Dann definiere $\pull(\Delta,R):=\pull(\pull(\Delta,R'),r_k))$ mit $R'=(r_1,\ldots,r_{k-1})$.

Sei $P$ ein Polytop und $\Delta$ eine Unterteilung von $P$. 
Sei $R$ die Menge der Ecken in $\Delta$. Dann heißt 
$\pull(\Delta,R)$  Pullingtriangulierung von $P$. 

\end{Definition}

Dies ist tatsächlich eine Trianguierung.


==> untersuchung_flusspolytope.tex <==
%
%
%

\section{Flusspolytope}

\subsection{$K_4$}
Der $K_4$ liefert ein höchstens $3$-dim Flusspolytop. Orientiere den $K_4$ und ordne die Knoten so auf 
einer Linie an, dass alle Pfeile nach rechts zeigen. Betrachte nun eine Zelle. Für den Bedarfsvektor 
$(b_1,b_2,b_3,b_4) \in \{0,1\}^4$ gilt dann:
\begin{displaymath}
%
\begin{array}{rclll}
-3 & \le & b_1 & \le & 0   \\ 
-2 & \le & b_2 & \le & 1 \\ 
-1 & \le & b_3 & \le & 2 \\ 
0  & \le & b_4 & \le & 3
\end{array}
\end{displaymath}
Da die Zellen volldimensional sind gilt sogar:
\begin{displaymath}
%
\begin{array}{rclll}
-2 & \le & b_1 & \le & -1   \\ 
-1 & \le & b_2 & \le & 0 \\ 
0 & \le & b_3 & \le & 1 \\ 
 1 & \le & b_4 & \le & 2
\end{array}
\end{displaymath}
(wäre eine der Abschätzungen oben scharf, wären damit automatisch Werte an drei Kanten klar, die anderen wären fest, wenn man eine Kante wählt, also die Zelle wäre 1-dimensional)
Insbesondere ist als $b_1 \le b_2 \le b3_ \le b4$

Es gibt also folgende volldimensionale Zellen: $Z_{(-2,-1,1,2)}$, $Z_{(-2,0,0,2)}$, $Z_{(-2,0,1,1)}$,
$Z_{(-1,-1,0,2)}$, $Z_{(-1,-1,1,1)}$, $Z_{(-1,0,0,1)}$ 

\[
Z_{(-2,-1,1,2)}
=
\begin{bmatrix}
 1 & 1 &  0 & 0 \\
 1 & 0 &  1 & 1\\
 0 & 1 &  1 & 1\\
 1 & 1 &  1 & 0\\
 1 & 1 &  0 & 1\\
 1 & 0 &  1 & 0 
\end{bmatrix}
\]
(erste drei Zeilen sind Kanten aus erstem Knoten raus, die nächsten zwei aus 2.tem Knoten und die letzte aus 3.tem Knoten, immer erste Kante zu nächstem Knoten)
Ist Simplex

$Z_{(-2,0,1,1)}$,
$Z_{(-1,-1,0,2)}$
sind nur 2-dim.

$Z_{(-2,0,0,2)}$,  $Z_{(-1,0,0,1)}$  sind Simplexe.

\[
Z_{(-1,-1,1,1)}=
\begin{bmatrix}
1 & 0 & 0 & 0 \\
0 & 1 & 1 & 0 \\
0 & 0 & 0 & 1 \\
1 & 0 & 1 & 1 \\
1 & 1 & 0 & 0 \\
0 & 0 & 1 & 0
\end{bmatrix}
\]
auch Simplex. Also sind Flusspolytope, die vom $K_4$ kommen (und allen Untergraphen) quadratisch erzeugt.

Frage: Lässt sich Theorem 14.8 aus Sturmfels auch auf Flusspolytope verallgemeinern?
